Unsupervised 3D out-of-distribution detection with latent diffusion models

Methods for out-of-distribution (OOD) detection that scale to 3D data are crucial components of any real-world clinical deep learning system. Classic denoising diffusion probabilistic models (DDPMs) have been recently proposed as a robust way to perform reconstruction-based OOD detection on 2D datasets, but do not trivially scale to 3D data. In this work, we propose to use Latent Diffusion Models (LDMs), which enable the scaling of DDPMs to high-resolution 3D medical data. We validate the proposed approach on near- and far-OOD datasets and compare it to a recently proposed, 3D-enabled approach using Latent Transformer Models (LTMs). Not only does the proposed LDM-based approach achieve statistically significant better performance, it also shows less sensitivity to the underlying latent representation, more favourable memory scaling, and produces better spatial anomaly maps. Code is available at https://github.com/marksgraham/ddpm-ood

==> figs/anomaly_maps.tex <==
\begin{figure}
% uncomment the fbox to help with trimming
%\fbox{
\includegraphics[trim={10 60 10 35},clip, width=0.7\textwidth]{figs/anomaly_maps.pdf}
%}
\centering
\label{fig:anomaly_maps}
\caption{Example anomaly maps for models based on 3- and 4-layer VQ-GANs. Maps for each model are shown on the same colour scale, but the scales vary between each model to obtain the best display for each model. Brighter regions are more anomalous.} 
\end{figure}
@article{hoogeboom2023simple,
  title={simple diffusion: End-to-end diffusion for high resolution images},
  author={Hoogeboom, Emiel and Heek, Jonathan and Salimans, Tim},
  journal={arXiv preprint arXiv:2301.11093},
  year={2023}
}
